Distributed Power Apportioning with Early Dispatch for Ancillary Services in Renewable Grids

This article develops a distributed framework for coordinating distributed energy resources (DERs) in a power network to provide secondary frequency response (SFR) as an ancillary service to the bulk power system. A distributed finite-time protocol-based solution is adopted that allows each DER in the network to determine power reference commands. The distributed protocol respects information exchange constraints posed by a communication network layer while being robust to delays in the communications channels. The proposed framework enables coordinated response and control of the aggregated DERs by apportioning the share of generation that each DER needs to provide towards meeting any specified global SFR command while allowing for adjustments due to variability in generation and demand in order to prioritize renewable energy sources in the network. A novel early dispatch mechanism with brown start is synthesized to achieve initial DER response to changing SFR commands that is faster than state-of-the-art distributed approaches. The proposed power apportioning protocol is validated using an end-to-end power hardware-in-the-loop configuration at a distribution system scale with 40+ physical hardware DERs, underlying 7-MW power system model, a 250-DER communication topology with physical and simulated distributed controller nodes, varied communication protocols, and an underlying real-world power system model. Experimental results demonstrate the efficacy of the proposed method toward distributed coordination of hundreds of DERs for providing fast response at SFR timescales.

==> definitions.tex <==
\begin{definition}(Cardinality of a set)
Let $A$ be a set. The cardinality of a set $A$ denoted by $|A|$ is a measure of the number of elements of the set $A$. 
\end{definition}
\begin{definition}(Undirected Graph)
% A directed graph (denoted as digraph) $\G$ is a pair $(\V,\E)$ where $\V$ is a set of vertices or nodes and $\E$ is a set of edges, which are ordered subsets of two distinct elements of $\V$. If an edge from $j \in \V$ to $i \in \V$ exists then it is denoted as $(i,j)\in \E$.  
An undirected graph $\G$ is a pair $(\V,\E)$ where $\V$ is a set of vertices or nodes and $\E$ is a set of edges such that for every pair of distinct nodes $i \in \V$ and $j\in \V$, if  $(i,j) \in \E$ then $(j,i) \in \E$.
\end{definition}


% \begin{definition}(Path) 
% In a directed graph, a directed path from node $i$ to $j$
% exists if there is a sequence of distinct directed edges of $\G$ of
% the form $(k_{1},i),(k_{2},k_{1}),...,(j,k_{m}).$
% \end{definition}
\begin{definition}(Strongly Connected Graph) A directed graph is strongly connected if it has a directed
path between each pair of distinct nodes $i$ and $j$.
\end{definition}
% \begin{definition}(Connected and Strongly Connected Graph) An undirected graph is connected if it has a path between each pair of distinct nodes $i$
% and $j$. A directed graph is strongly connected if it has a directed
% path between each pair of distinct nodes $i$ and $j$.
% \end{definition}
% \begin{definition}(In-neighbor and out-neighbor of node) Given a directed graph $G=(\V,\E)$, a node $j \in \V$ is said to be an in-neighbor or out-neighbor of node $i\in \V$ if $(i,j) \in \E$ or $(j,i) \in \E$ respectively. % \end{definition}
\begin{definition}(Column Stochastic Matrix) A real $n\times n$ matrix $A=[a_{ij}]$ is called a column stochastic matrix if $1 \geq a_{ij} \geq 0$ for $1\leq i,j\leq n$ and $\displaystyle \sum_{i=1}^{n}a_{ij}=1$ for $1\leq j\leq n.$ 
\end{definition}
\begin{definition}(Irreducible Matrix)
	A $N \times N$ matrix $A$ is said to be irreducible if for any $i, j \in \{1,...,N\}$, there exist $m \in \mathbb{N}$ such that $(\textbf{A}^m)(i,j) > 0$, that is, it is possible to reach any state from any other state in a finite number of hops.
\end{definition}
\begin{definition}(Primitive Matrix) A non negative matrix $A$ is primitive if it is irreducible and has only one eigenvalue of maximum modulus. 
\end{definition}
% \begin{definition}(Undirected Graphs)
% 	An undirected graph $\G$ is a pair $(\V,\E)$ where $\V$ is a set of vertices or nodes and $\E$ is a set of edges or arcs, which are unordered subsets of two distinct elements of $\V$, that is, $(i,j) \in \E$ (edge from node $j \in \V$ to node $i \in \V$) implies $(j,i)\in \E$ (edge from node $i \in \V$ to node $j \in \V$).   
% \end{definition}

\begin{definition}(Neighbor Set)
	Given an undirected graph $\G=(\V,\E)$ and a node $j\in~\V$, the neighbor set of $j$ is defined as
	$\mathcal{N}_j:=\{i| (j,i) \in \E \ \text{or} \ (i,j) \in \E\}.$ In the context of this paper, information exchange is possible between node $j$ and members of $\mathcal{N}_j$. We assume that information can flow in both directions along an undirected edge.  
	\end{definition}
\begin{definition}(In-neighbor Set and Out-neighbor Set)
In a graph $\G:=(\V,\E)$, the in-neighbor set, $\mathcal{N}_j^{-}$,  and out-neighbor set, $\mathcal{N}_j^+$, of node $j \in \V$, are given as $\mathcal{N}_j^{-}:=\{i| (j,i)$ $ \in \E, i \neq j\}$ and $\mathcal{N}_j^{+}:=\{i| (j,i)$ $ \in \E, i \neq j\}$ respectively. The cardinalities of the in-neighbor set and out-neighbor set of a node $i \in \V$ are called the in-degree  ($D_{i}^{-}$) and out-degree of the node ($D_{i}^{+}$) respectively. 
\end{definition}
% \begin{definition}(Out-neighbor Set)
% In a graph $\G:=(\V,\E)$, the out-neighbor set ${N}_j^{+}$ of node $j \in \V$, ${N}_j^{+}:=\{i| (i,j) \in \E, i \neq j\}.$ The cardinality of the out-neighbor set of a node $i \in \V$ is called out-degree of the node and is denoted as $D_{i}^{+}$.
% \end{definition}

\begin{definition}(Diameter of a Graph)
The diameter $D$ of an undirected graph $\G=(\V,\E)$ is defined as the longest shortest path between any two nodes in the network. 
\end{definition}
